Quantum oscillations of the nonlinear planar effects signifying chiral anomaly in Weyl Semimetals

In view of searching the signature of the celebrated chiral anomaly (CA) in Weyl semimetals (WSMs) in ongoing experiments, quantum oscillation in linear response regime has been considered as an important signature in the magneto transports in WSMs, due to its unique relation to CA. Investigating the nonlinear planar effects (NPEs) starting from the semiclassical regime to the ultra-quantum limit within the framework of Boltzmann transport theory incorporating Landau quantization, we here propose the quantum oscillations in NPEs can serve as a robust signature of CA in WSMs. By obtaining analytical expressions, we show that the quantum oscillations of the nonlinear effects exhibit two different period scales in 1/B (B is the magnetic field) compared to the linear responses where only one period scale exists. We find that these quantum oscillations in NPEs are attributed to the deviation of chiral chemical potential (CCP), which is proportional to the finite band tilt as well as transverse electric field and therefore, directly linked to CA in WSMs. In addition, we also show that the CA-induced nonlinear magneto conductivity is linear and independent in the magnetic field in the semiclassical and ultraquantum regimes, respectively. We conclude that the proposed behaviors of NPEs in different regimes uniquely signify the existence of CA and therefore, can serve as a probe of identifying CA in WSMs in experiments.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );
 
        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );
 
        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
 
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
